Build It, Break It, Fix It: Contesting Secure Development

Typical security contests focus on breaking or mitigating the impact of buggy systems. We present the Build-it Break-it Fix-it BIBIFI contest which aims to assess the ability to securely build software not just break it. In BIBIFI teams build specified software with the goal of maximizing correctness performance and security. The latter is tested when teams attempt to break other teams submissions. Winners are chosen from among the best builders and the best breakers. BIBIFI was designed to be open-ended - teams can use any language tool process etc. that they like. As such contest outcomes shed light on factors that correlate with successfully building secure software and breaking insecure software. During we ran three contests involving a total of teams and two different programming problems. Quantitative analysis from these contests found that the most efficient build-it submissions used CC but submissions coded in a statically-typed language were less likely to have a security flaw build-it teams with diverse programming-language knowledge also produced more secure code. Shorter programs correlated with better scores. Break-it teams that were also build-it teams were significantly better at finding security bugs.

==> Makefile <==
TARGET   = paper
TEXFILES = $(wildcard *.tex)
FIGURES  = 

PS2PDF_FLAGS=-dCompatibilityLevel=1.4 -dUseCIEColor -dMaxSubsetPct=100 -dSubsetFonts=true -dOptimize=true -dEmbedAllFonts=true -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dAutoFilterGrayImages=false -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode -dMonoImageFilter=/FlateEncode 

.SUFFIXES:	.plot .eps .fig

all: $(TARGET).pdf

figures/%.eps: plots/%.plot
	gnuplot $< > $@

graphs: $(addprefix figures/, $(addsuffix .eps, $(FIGURES)))

$(TARGET).aux: $(TEXFILES) 
	pdflatex $(TARGET).tex

$(TARGET).bbl: $(TARGET).aux
	bibtex $(TARGET)

## $(addsuffix .eps, $(FIGURES)) 

$(TARGET).pdf: graphs $(TARGET).bbl
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex

nobib:: $(addsuffix .eps, $(FIGURES)) $(TARGET).aux
	dvips $(TARGET).dvi -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -o $(TARGET).ps
	ps2pdf ${PS2PDF_FLAGS} $(TARGET).ps

view:: $(TARGET).pdf
	open $(TARGET).pdf

see:: $(TARGET).dvi
	xdvi $(TARGET)

%.eps: plots/%.plot
	gnuplot $< > figures/$@

%.eps: figures/%.fig
	fig2dev -L eps -p dummy $< $*.eps

spell::
	ispell *.tex

clean::
	rm -fv *.dvi *.aux *.log *~ *.bbl *.blg *.toc *.ps *.pdf *.ent parsetab.py
	rm -fv $(addprefix figures/, $(addsuffix .eps, $(FIGURES)))

fresh::
	rm -fv *.dvi *.aux *.log *~ *.bbl *.blg *.toc *.ps *.pdf

distclean:: clean
	rm $(TARGET).ps

# piotr's build, independent of anything above
DEP := *.tex *.bib figures/*.pdf figures/*.tex
DEP := $(foreach i,$(DEP),$(shell ls $(i) 2> /dev/null))
watch: $(DEP)
	perl watch.pl watch quietly $(DEP)
quietly:
	perl watch.pl render_latex paper "\input{paper.tex}"


==> figures/Makefile <==
-include ../Makefile.common

ACTIVE := summary_data

FIGURES := \
	summary_system \
	summary_data \

start:
	make open
	make watch

all: $(FIGURES:=%.pdf)
	mv *.pdf figures

open:
	make open-$(ACTIVE)

watch:
	make watch-$(ACTIVE)

ALL_TARGETS :=
define FIG_RULES
ALL_TARGETS += $1.pdf
$1 :
	make start-$1
start-$1 :
	make open-$1
	make watch-$1
$1.rendered.pdf : $1.pdf
	@cp $1.pdf $1.rendered.pdf
$1.pdf : $1.tex *.pdf
	perl ../watch.pl render_latex $1 "\input{$1.tex}"
open-$1 : $1.rendered.pdf
	$(OPEN) $1.rendered.pdf
watch-$1 :
	perl ../watch.pl watch $1.rendered.pdf $1.tex *.pdf
endef

$(foreach fig,$(FIGURES),$(eval $(call FIG_RULES,$(fig))))

clean:
	rm -Rf *.aux *.lof *.log *.lot *.bbl *.blg *.toc *.out *.bcf *.synctex.gz; true
	rm -Rf *~; true
	rm -Rf $(ALL_TARGETS) $(FIGURES:%=%.rendered.pdf); true
	rm -Rf .DS_Store; true
	rm -Rf .iTeXMac; true
	rm -Rf *.*.gz; true
	rm -Rf *.pdfsync; true
	rm -Rf *.synctex; true


==> old-intro.tex <==
%\mwh{Need introductory paras here; some are commented out below.}

% \mwh{I think we want to change the tack of the intro to downplay the
%   generalization possibilities of contest outcomes. Otherwise we will
%   disappoint.}

\pxm{Try not to use ``experts''?:} Experts have long advocated that achieving security in a computer
system requires treating security as a first-order design
goal~\cite{SaltzerSc75}.
%
%% Over the last decade, Microsoft~\cite{securecode,sdl} and
%% others~\cite{bss,buildsecin,csslp} have described processes and methods
%% for building secure software, and researchers and companies have
%% developed myriad software analysis and testing
%% tools~\cite{fortify,coverity,lapse} to help developers find
%% vulnerabilities. Despite these efforts,
%
Despite proposals of new methods for building secure
software~\cite{securecode,sdl,bss,buildsecin,csslp}, myriad software
analysis and testing tools~\cite{fortify,coverity,lapse} to help
developers find vulnerabilities, and billions spent annually on
security~\cite{costcybercrime}, 
%
the situation seems to have
worsened, not improved, with vulnerable software proliferating.
\pxm{citation needed for last claim}
%% despite billions spent annually on security~\cite{costcybercrime}.

% This disconnect between secure development innovation and marketplace
% adoption may be due to a lack of \emph{evidence}. In particular, no one
% would disagree that certain technologies, such as type-safe programming
% languages and static analysis tools, and activities, such as code
% reviews and penetration testing, can improve software's security. The
% question is how \emph{effective} these (and other) things are, in terms
% of their costs vs.~benefits. Companies would like to know: Which
% technologies or processes shake out the most (critical) bugs? Which are
% the easiest to use? Which have the least impact on other metrics of
% software quality, such as performance and maintainability?  It is
% currently difficult to answer these questions because we lack the empirical
% evidence needed to do so.

%% Despite an increased attention towards making security a first-order
%% design
%% goal~\cite{SaltzerSc75,gatesmemo,securecode,sdl,bss,buildsecin,csslp},
%% and despite billions spent annually on security~\cite{costcybercrime},
%% developers continue to produce insecure software.

%% Though this situation may improve with better tools and design
%% principles, we note that they are only effective if developers use them
%% and use them well.
%
Better tools and design principles are only effective if developers use
them and use them well.
%
%Rather,
Thus, to enable more secure software, we must first answer a critical
question: \emph{What tools, backgrounds, and best practices make
  developers most effective at developing secure software?} 
\pxm{most effective or just effective?}


Unfortunately, there is very little \emph{empirical evidence} about
what techniques developers currently use when developing secure
software.
%
As a result, when developing new tools or new education curricula
regarding secure development, we can rely only on anecdotal
evidence---for example, many advocate avoiding C and programming in
higher-level programming languages\pxm{citation needed}, but how significant an effect does
this actually have on a program's security?


In this paper, we seek to develop the first steps towards being able to
obtain empirical data about the effects that various practices, tools,
and programmer experience have on a group's ability to build and find
bugs in secure software.
%
Our insight is that a \emph{secure programming competition}, if
designed carefully, can be used as a \emph{controlled experiment} that
gives researchers \emph{in situ} data on how teams develop code, while
also enticing participation and exposing a new group of developers to
secure programming. 
\pxm{The enticing new developers thing might go contrary to answering
  the critical question mentioned in the previous column, new
  developers would not be using best practices. 
  Could they be used as a control against which to judge already
  well-versed developers?}




%% There are many anecdotal observations on what makes developers
%% effective at writing secure software---for example, a long-held
%% hypothesis among advocates of higher-layer programming languages is
%% that programming in C leads to greater security vulnerabilities.
%% %
%% Yet there is surprisingly little \emph{empirical evidence}, owing
%% largely to the fact that there are no large-scale \emph{controlled
%% studies} of secure programming.
%% %
%% Running a controlled study at scale has proven daunting; to do so in
%% industry, for example, would require costly, duplicate effort by
%% different teams.
%% %
%% We present a novel approach to performing large-scale, controlled
%% studies of best secure practices: a secure programming competition.


%% One can easily perform a post hoc analysis of a particular body of
%% code---particularly after a vulnerability has been released---but to
%% reason about best practices at large, one must be able to look at a
%% wide range of teams,


%% While there have been many anecdotal answers to this question, we find
%% that there is surprisingly little \emph{empirical evidence}  on what
%% makes developers effective at writing secure software in practice.



%% We believe this situation arises, at least in part, from a lack of an
%% \emph{empirical evidence} of what techniques, backgrounds, and best
%% practices work well when developing secure software in practice.
%% 
%% 
%% For example, code reviews, penetration testing, and static code
%% analysis are all known to improve security by finding vulnerabilities.
%% But the relative costs and benefits of these techniques are largely
%% unknown, which leaves educators and policymakers in a bind: they may
%% believe that secure coding is important, but they do not know which
%% ideas are fundamental, so they are unsure, given limited time, what to
%% invest in and teach.  


%% This paper presents a novel means of collecting empirical data about
%% best secure-programming practices: a 
%
%% We present \textbf{Build-it, Break-it, Fix-it} (\bibifi), a new
%% software security contest whose focus is on \emph{building secure
%% systems}.
%% %
%% %% , and data collected from two large-scale runs of the competition.
%% %
%% \bibifi takes inspiration from popular capture-the-flag
%% (CTF) cybersecurity contests \cite{nationalccdc,defconctf,csawctf} and
%% from programming contests \cite{topcoder,acmprogramming,icfpcontest},
%% but is unique in that it combines ideas from both in a novel way.
%
% Although no contest can truly capture the many difficulties of
% professional development, we hope it will provide some general
% insight nevertheless, and thus provide some sorely needed evidence
% about what works for building secure software.

% BIBFI contestants build secure software, and/or identify security
% problems in software built by other contestants. 
%% A \bibifi contest has three phases. The first phase, \emph{Build-it},
%% asks small development teams to build software according to a provided
%% specification including security goals. The software is scored for
%% being correct, efficient, and feature-ful. The second phase,
%% \emph{Break-it}, asks teams to find defects in other teams' build-it
%% submissions. Reported defects, proved via test cases, benefit a
%% Break-it team's score and penalize the Build-it team's score; more
%% points are assigned to security-relevant problems. (A team's break-it
%% and build-it scores are independent, with prizes for top scorers in
%% each category.)  The final phase, \emph{Fix-it}, asks builders to fix
%% bugs and thereby get points back if the process discovers that distinct
%% break-it test cases identify the same underlying defect.  During all
%% phases, we collect data on the processes and tools the contestants use
%% to build and assess software. These include the version control history
%% for the developers, and demographic information for all participants.
%% %activity logs for all participants.
%% %% After the contests, we will analyze these data to learn how contestants
%% %% approach secure programming, and what bugs are common (or overlooked).

We designed \bibifi to give researchers \emph{in situ} data on how
teams develop code---for better or for worse---when security is a
first-order design goal.
%
As such, \bibifi contestants are afforded a significant amount of
freedom. Build-it teams can choose to build their software using
whatever programming language(s), libraries, tools, or processes they
want, and likewise break-it teams can hunt for vulnerabilities as they
like, using manual code reviews, analysis or testing tools, reverse
engineering, and so on. During the contest, we collect data on each
team's activities. For example, we keep track of commit logs, testing
outcomes, and interactions with the contest site. Prior to and after
the contest, we survey the participants to record their background,
mindset, choices, and activities.
%
By correlating \emph{how} teams worked with \emph{how well} they
performed in the competition, we can gain insight into what practices
do and do not work.

%% By correlating \emph{how} teams worked with \emph{how well} they
%% performed in the competition, researchers can learn about what
%% practices do and do not work.  Treating the contest as a scientific
%% experiment, the contest problem is the control, the final score is the
%% dependent variable, and the various choices made by each team, which we
%% observe, are the independent variables.
%% %
%% To permit repeatable, statistically significant results, we have
%% designed \bibifi and implemented its infrastructure to scale to 
%% multiple competitions with thousands of competitors.


To demonstrate the utility of \bibifi, and to gain initial empirical
insight into what practices lead to more secure development, we present
a rigorous quantitative and qualitative analysis of data we collected
from two large-scale competitions we held in 2015.
%
These competitions comprised 421 total participants (201 teams) from
over a dozen countries; of these, 301 participants (116 teams)
completed the contest.
%
Most of the participants were part of a MOOC (Massive Online Open
Courseware) course on cybersecurity, and had thus been recently exposed
to concepts of secure software and cryptography; we therefore believe
that they are largely representative of the population of professional
developers. \pxm{Are you really claiming that students only recently
  exposed to these security topics are representative of professional developers??!?!?}
%
In our particular runs of \bibifi, we focused on gathering evidence on
broad effects on build-it and break-it teams' scores---including the
type of programming language used, team size, and participant
experience---and our results demonstrate several interesting,
statistically significant effects. For example, using C/C++ increased
performance, but also increased chances of a security bug found in
code; teams with broader programming language experience and who wrote
shorter programs also produced more secure implementations. On the
flip side, larger teams found more bugs during the break-it phase, and
knowledge of C and programming experience were also correlating
(though not statistically significant) factors\pxm{correlating to what?}. Teams that also
participated during the build-it phase were significantly more likely
to find a security bug than those that did not. 
%
\pxm{Of all of the sentences so far, this is my least favorite:} We also examined submissions qualitatively and report on interesting
things we found.\footnote{This paper subsumes a
  previously published 6-page workshop paper~\cite{bibifi-cset15}. The
  basic \bibifi design and implementation also appeared in that paper,
  as did a brief description of a pilot run of the contest
  involving 12 teams. This paper presents many more details about the
  contest setup; describes two new contest runs, in Spring'15 and
  Fall'15, involving more than 200 teams; and carries out a detailed
  quantitative and qualitative analysis of data gathered from those runs.}

We emphasize that the results we present in this paper are a first step
towards developing an empirical understanding of what helps and hurts
secure software development.
%
There are many interesting questions that even our moderately large
competitions would not be able to answer in a statistically significant
way.
%
%% In making \bibifi's infrastructure publicly available, we hope that
%% this opens up a line of research built on running controlled
%% experiments of secure programming methodologies.
%
We will be making the \bibifi code and infrastructure publicly
available so that others may run their own competitions; we hope that
this opens up a line of research built on controlled experiments of
secure programming methodologies.

The rest of this paper is organized as follows.
%
We present the design of \bibifi in~\S\ref{sec:contest} and describe
the specifics to the contests we ran in~\S\ref{sec:contests}.
%
We present the quantitative analysis of the data we collected from
these contests in~\S\ref{sec:analysis}, and qualitative analysis
in~\S\ref{sec:stories}.
%
We review related work in~\S\ref{sec:related} and conclude
in~\S\ref{sec:conclusions}.

%% This paper makes two broad contributions.
%% %
%% \emph{First}, it describes the design and implementation of \bibifi
%% (\S\ref{sec:contest}), which applies novel scoring techniques to ensure
%% that high scores in the contest correlate with 
%% %and the contest infrastructure (~\S\ref{sec:implementation}), 
%% %% focusing on how
%% %% both aim to ensure that high scores in the contest correlate with
%% meaningful, real-world outcomes.
%% %
%% \emph{Second}, it describes two runs of the contest
%% (\S\ref{sec:contests}) we held during 2015, and presents a rigorous
%% quantitative (\S\ref{sec:analysis}) and qualitative
%% (\S\ref{sec:stories}) analysis of the data we collected from these
%% contests.
%% %This paper discusses 
%% %
%% % collected from two runs of the contest carried out during 2015.
%% %
%% Most contest participants were part of a Capstone project in a Coursera
%% specialization on Cybersecurity.  These contestants have familiarity
%% with software security and cryptography, as those courses (delivered
%% through Coursera) are pre-requisites to participate in the capstone
%% exercise.  As a result, we believe the participants from these contests
%% are largely representative of the population of professional
%% developers, but we discuss potential limitations of our
%% study in~\S\ref{sec:limitations}.
%% 
%% \mwh{More here on what we found.}
%% 
% \paragraph*{Contributions}

%% This paper makes two main contributions.
%% %
%% \emph{First}, it describes the design and implementation of \bibifi
%% (~\S\ref{sec:contest}), which applies novel scoring techniques to
%% ensure that high scores in the contest correlate with 
%% %and the contest infrastructure (~\S\ref{sec:implementation}), 
%% %% focusing on how
%% %% both aim to ensure that high scores in the contest correlate with
%% meaningful, real-world outcomes.
%% %
%% \emph{Second}, we present a detailed analysis of data we gathered from
%% two separate \bibifi competitions.
%% %

%% Our results provide an empirical basis that we hope guides future
%% development of new tools, techniques, and educational curricula.
%% %
%% %% One of our findings is that, in general, a group with more programming
%% %% experience is better not only at writing secure code, but also breaking
%% %% others' code.
%% %
%% We have designed \bibifi so that it can be run by other groups, and we
%% intend to make our code, data, and infrastructure freely available for
%% future researchers and practitioners to use.

%\mwh{Add some tidbits here, to tantalize the reader}

% For example, we want broad participation to acquire more data, leading
% to more convincing conclusions. As such we must deal with issues of
% scale, in particular, minimizing the role of human judges. The Fix-It
% phase supports this goal. In particular, we want to reduce the
% likelihood that a build-it team's score is unduly penalized by having
% a single vulnerability's impact magnified by its being found
% repeatedly, but via superficially different test cases. We could ask
% human judges to look at all of these test cases, but this will not
% scale. Instead, we ask human judges to look at a team's bugfix, and to
% judge whether it truly fixes a single bug. Assuming that m
% More participants
% will produce more experimental data and hopefully statistically
% significant outcomes, e.g., avoiding a misattribution of success to a
% technique that would show its true colors if put to a stronger test.
% This means that we
% want to reduce the likelihood that a build-it team's high score owes
% to break-it teams simply not looking at it to find bugs. 

